Effects of Gauss-Bonnet gravity on thermodynamics of (3+1)$-D$ AdS black holes

We studied the thermodynamics of the black holes with Gauss-Bonnet correction term in $3+1-$ dimensional AdS spacetime. It is known that the term has no effect on the equation of motion, however, it modifies the entropy formula of Wald as it has an effect of the Gauss-Bonnet parameter term. We studied charged black holes, namely, Reissner-Nordstr\"{o}m and Born-Infeld under this regime. We encountered divergences in heat capacity. After eliminating the possibility of first order phase transition, we applied two well trusted methods from standard thermodynamics, namely, Ehrenfest scheme and Ruppeiner's state space geometry analysis to ensure the second order nature of phase transition points. Effects of Gauss-Bonnet and Born-Infeld parameter are also discussed.

==> Untitled Folder/umbclogo-2003-01.tex <==
% UMBC logo
%
% This file is \included in PPRumbc*.sty
%
% Rouben Rostamian
% September 2002

\definecolor{shadowcolorA}{gray}{0.7}
\definecolor{shadowcolorB}{gray}{0.2}
\newcommand{\umbclogo}{%
	{\fontfamily{phv}\fontseries{b}\fontshape{sl}\fontsize{7}{7}%
	\selectfont%
	\makebox[0pt][l]{\raisebox{-0.20ex}[0pt][0pt]{\color{shadowcolorA}\hspace*{.20ex}UMBC}}%
	\makebox[0pt][l]{\raisebox{-0.10ex}[0pt][0pt]{\color{shadowcolorB}\hspace*{.10ex}UMBC}}%
	{\red UMBC}\hspace{.20ex}%
}}

% Define custumized bullets if the tribullet.sty package is available.
\IfFileExists{tribullet.sty}{
	\RequirePackage{tribullet}
	\myitem{1}{\raisebox{0.60ex}{\tribullet[1.40ex]{red}}}
	\myitem{2}{\raisebox{0.55ex}{\tribullet[1.30ex]{blue}}}
	\myitem{3}{\raisebox{0.50ex}{\tribullet[1.25ex]{cyan}}}
}{}


==> umbclogo-2003-01.tex <==
% UMBC logo
%
% This file is \included in PPRumbc*.sty
%
% Rouben Rostamian
% September 2002

\definecolor{shadowcolorA}{gray}{0.7}
\definecolor{shadowcolorB}{gray}{0.2}
\newcommand{\umbclogo}{%
	{\fontfamily{phv}\fontseries{b}\fontshape{sl}\fontsize{7}{7}%
	\selectfont%
	\makebox[0pt][l]{\raisebox{-0.20ex}[0pt][0pt]{\color{shadowcolorA}\hspace*{.20ex}UMBC}}%
	\makebox[0pt][l]{\raisebox{-0.10ex}[0pt][0pt]{\color{shadowcolorB}\hspace*{.10ex}UMBC}}%
	{\red UMBC}\hspace{.20ex}%
}}

% Define custumized bullets if the tribullet.sty package is available.
\IfFileExists{tribullet.sty}{
	\RequirePackage{tribullet}
	\myitem{1}{\raisebox{0.60ex}{\tribullet[1.40ex]{red}}}
	\myitem{2}{\raisebox{0.55ex}{\tribullet[1.30ex]{blue}}}
	\myitem{3}{\raisebox{0.50ex}{\tribullet[1.25ex]{cyan}}}
}{}

